Relative cohomology theory for profinite groups

In this paper we define and develop the theory of the cohomology of a profinite group relative to a collection of closed subgroups. Having made the relevant definitions we establish a robust theory of cup products and use this theory to define profinite Poincar\'e duality pairs. We use the theory of groups acting on profinite trees to give Mayer-Vietoris sequences, and apply this to give results concerning decompositions of 3-manifold groups. Finally we discuss the relationship between discrete duality pairs and profinite duality pairs, culminating in the result that profinite completion of the fundamental group of a compact aspherical 3-manifold is a profinite Poincar\'e duality group relative to the profinite completions of the fundamental groups of its boundary components.

==> GrpExtensions.tex <==

\section{Group Extensions}
In this section we will note that the usual spectral sequence for group extensions extends to relative cohomology in the expected fashion. First we state a stronger criterion for a module to have type FP$_\infty$. This is a slight rephrasing of a criterion due to Pletch \cite{Pletch80a}, which only holds in the category of $\Zpof{G}$-modules for $p$ a prime. 
\begin{theorem}[Theorem 1.6 of \cite{Pletch80a}]\label{PletchFPn}
Let $G$ be a profinite group and let $M$ be a finitely generated module in \Gmod[p]{C}. Then the following are equivalent.
\begin{itemize}
\item $\Ext^k_G(M, A)$ is finite for all $A\in\Gmod[p]{F}$ and all $k\leq n$
\item There is a resolution $P_\bullet\to M$ in \Gmod[p]{C} with $P_k$ finitely generated and projective for $k\leq n$.
\end{itemize}
\end{theorem}
\begin{rmk}
The second property is of course the FP$_n$ condition. But since in \cite{Pletch80a} the term `FP$_n$' is defined by the first property it seemed better to spell things out.
\end{rmk}
We also recall that the Lyndon-Hochschild-Serre spectral sequence holds in the world of profinite groups.
\begin{prop}[see Theorem 7.2.4 of \cite{RZ00}]\label{LHS1}
Let $G$ be a profinite group and $N$ a closed normal subgroup of $G$ with $G/N=Q$. For $A\in\Gmod[\pi]{D}$ there is a natural convergent first quadrant cohomological spectral sequence
\[E_2^{rs}=H^r(Q, H^s(N; A))\Rightarrow H^{r+s}(G,A) \]
\end{prop}
\begin{prop}
Let $(G,\famS)$ be a profinite group pair where $\famS$ is continuously indexed by a profinite space $X$ and let $N$ be a closed normal subgroup of $G$ contained in $S$ for all $S\in\famS$. Let $Q=G/N$ and let ${\cal T}=\{S/N\mid S\in\famS\}$ be a family of subgroups of $Q$; then $\cal T$ is continuously indexed by $X$. The group $N$ acts trivially on $\Delta_{G,\famS}$ and $\Delta_{G,\famS}$ (regarded as a $Q$-module) is naturally isomorphic to $\Delta_{Q,\cal T}$.
\end{prop}
\begin{proof}
The statement that $\cal T$ is continuously indexed follows immediately from the definition. For $x\in G$, $n\in N$, $S\in\famS$ the formula
\[n\cdot xS=xx^{-1}nxS=xS \]
shows that $N$ acts trivially on $\Zpof{G/\famS}$, hence on $\Delta_{G,\famS}$. Finally the natural continuous bijections $G/S\iso (G/N)/(S/N)$ show that $\Zpof{G/\famS}$ is naturally isomorphic as a $G$-module to $\Zpof{Q/\cal T}$ in a way compatible with the augmentation to \Z[p]. Hence  $\Delta_{G,\famS}$ is naturally isomorphic to $\Delta_{Q,\cal T}$.
\end{proof}

\begin{prop}\label{LHS2}
Let $(G,\famS)$ be a profinite group pair and let $N$ be a closed normal subgroup of $G$ contained in $S$ for all $S\in\famS$. Let $Q=G/N$ and let ${\cal T}=\{S/N\mid S\in\famS\}$. For $A\in\Gmod[\pi]{D}$ there is a natural convergent first quadrant cohomological spectral sequence
\[E_2^{rs}=H^r(Q,{\cal T}; H^s(N; A))\Rightarrow H^{r+s}(G,\famS; A) \]
\end{prop}
\begin{proof}
This follows from the spectral sequence in Proposition \ref{LHS1} via the natural isomorphism
\[H^s(N; \Hom(\Delta, A)) = \Hom(\Delta, H^s(N, A)) \]
where $\Delta=\Delta_{G,\famS}$. This isomorphism holds because $\Delta$, viewed as an $N$-module, is simply a free \Z[p]-module with trivial $N$-action. Hence the functor $\Hom(\Delta, -)$ is an exact functor with
\[ \Hom_N(P, \Hom(\Delta, A)) = \Hom(\Delta, \Hom_N(P,A))\]  
(as $G$-modules) for every $P\in \mathfrak{C}_p(N)$ and the cohomology isomorphisms follow.
\end{proof}

\begin{prop}\label{LHSFPn}
Let $(G,\famS)$ be a profinite group pair and let $N$ be a closed normal subgroup of $G$ contained in $S$ for all $S\in\famS$. Let $Q=G/N$ and let ${\cal T}=\{S/N\mid S\in\famS\}$. Assume that $N$ and $(Q,\cal T)$ have type \pFP[\infty]. Then $(G,\famS)$ has type \pFP[\infty].
\end{prop}
\begin{proof}
This follows immediately from the above spectral sequence and Theorem \ref{PletchFPn}.
\end{proof}

\begin{prop}\label{LHSPDn}
Let $(G,\famS)$ be a profinite group pair and let $N$ be a closed normal subgroup of $G$ contained in $S$ for all $S\in\famS$. Let $Q=G/N$ and let ${\cal T}=\{S/N\mid S\in\famS\}$. Assume that $N$ is a PD$^n$ group at the prime $p$ and $(Q,\cal T)$ is a PD$^q$ pair at the prime $p$. Then $(G,\famS)$ is a PD$^{n+q}$ group with dualising module
\[I_p(G, \famS)=  I_p(N)\otimes I_p(Q, \cal T)\]
where $G$ acts on $I_p(N)$ via the conjugation action on $N$ and naturality and on $I_p(Q, \cal T)$ via the quotient map $G\to Q$.
\end{prop}
\begin{proof}
By the previous proposition the pair $(G,\famS)$ is of type \pFP[\infty]. Since $\cd_p(N)=n$ and $\cd_p(Q, {\cal T})=q$ the spectral sequence in Proposition \ref{LHS2} immediately forces $\cd_p(G,\famS)\leq n+q$. It only remains to verify that this inequality is an equality and that the dualising module has the claimed form. We have, for each $r$ and $s$ and each $A\in\Gmod[p]{D}$, the following chain of isomorphisms induced by cup products.
\begin{eqnarray*}
H^r(Q,{\cal T}; H^s(N,A))& \iso & H^r\left(Q,{\cal T}; H^{n-s}(N, \Hom(A, I_p(N)))^\ast  \right)\\
&\iso & H^{q-r}\left(Q, \Hom\left(H^{n-s}(N, \Hom(A, I_p(N)))^\ast, I_p(Q,{\cal T})\right) \right)^\ast\\
&\iso & H^{q-r}\left(Q, \Hom\left( D_p(Q,{\cal T}), H^{n-s}(N, \Hom(A, I_p(N)))\right) \right)^\ast\\
&\iso & H^{q-r}\left(Q, H^{n-s}\left(N,\Hom( D_p(Q,{\cal T}), \Hom(A, I_p(N)))\right) \right)^\ast\\
&\iso & H^{q-r}\left(Q, H^{n-s}\left(N,\Hom( A, I_p(N)\otimes I_p(Q,{\cal T}) )\right) \right)^\ast
\end{eqnarray*}
where the only non-trivial isomorphism is that between the third and fourth line, which follows because $D_p(Q,\cal T)$ is isomorphic to the trivial module $\Z[p]$ as an $N$-module. Now the cup product maps are defined on the level of chains and are natural with respect to chain maps. The maps on the first page of the spectral sequence are simply chain maps, hence are natural with respect to the cup product and the isomorphisms above are natural isomorphisms of spectral sequences and converge to an isomorphism
\[ H^{r+s}(G, \famS; A) \iso H^{q-r+n-s}\left(G, \Hom(A, I_p(N)\otimes I_p(Q,{\cal T}) )\right) \]
which, by the naturality properties explained above and standard theory of spectral sequences, is actually the map induced by the cup product on $G$. The proof is complete.
\end{proof}
The converse to this (as in Theorem 7.3(ii) of \cite{BE77}) is surely true, but our techniques are not quite sufficient to prove this. In the classical theory this proceeds via the Bieri-Eckamnn criterion \cite{BE74}, but there seems to be no immediate way to extend this criterion to the world of profinite groups.

